Dynamic Epistemic Logic with ASP Updates: Application to Conditional Planning

Dynamic Epistemic Logic (DEL) is a family of multimodal logics that has proved to be very successful for epistemic reasoning in planning tasks. In this logic, the agent's knowledge is captured by modal epistemic operators whereas the system evolution is described in terms of (some subset of) dynamic logic modalities in which actions are usually represented as semantic objects called event models. In this paper, we study a variant of DEL, that wecall DEL[ASP], where actions are syntactically described by using an Answer Set Programming (ASP) representation instead of event models. This representation directly inherits high level expressive features like indirect effects, qualifications, state constraints, defaults, or recursive fluents that are common in ASP descriptions of action domains. Besides, we illustrate how this approach can be applied for obtaining conditional plans in single-agent, partially observable domains where knowledge acquisition may be represented as indirect effects of actions.

==> background.tex <==
%!TEX root = main.tex

\

\section{Dynamic Epistemic Logic}


In this section, we review the basic notions of Dynamic Epistemic Logic~(DEL) that weill be needed in the rest of the paper.
We mainly follow the presentation given in~\cite{AndersenBJ12,BolanderA11},
with a slightly generalisation: we allow the dynamic operator to be applied to abstract \emph{updating objects}
rather than just \emph{event models}.
Then, the usual DEL approach with event models~\cite{BatlagMS98} is just a particular case in which those
updating objects are event models.
On the other hand, this generalisation allow us to introduce DEL[ASP] as a particular case of DEL in which the updating objects are logic programs.
Formally, given a set of propositional symbols~$\at$ and a set of updating objects~$\uobj$,
a \emph{(dynamic epistemic) formula}
% or just \emph{\DEformula}
$\varphi$ is defined according to the following grammar:
\begin{gather*}
\varphi ::=  \bot \mid p \mid \varphi \wedge \varphi \mid \varphi \vee \varphi \mid \varphi \to \varphi \mid \sneg \varphi \mid \bK \varphi \mid [o] \varphi
\end{gather*}
where $p \in \at$ is a proposition and $o \in \uobj$ and updating object.
The operator~$\bK$ is the epistemic modality and, intuitively, a formula~$\bK \varphi$ means that ``the (planning) agent knows $\varphi$.''
The symbol~``$\sneg\,$'' stands here for classical negation (we reserve the symbol~``$\neg$'' for intuitionistic negation latter on).
A formula~$\varphi$ is called \emph{objective} if the operator $\bK$ does not occur in it.
It is called \emph{subjective} if it has at least some proposition and every proposition is in the scope of the epistemic operator~$\bK$.
As usual,
we define the following abbreviations:
$\fF \leftrightarrow \fG \eqdef (\fF \to \fG) \wedge (\fG \to \fF)$,
\ $(\fF \leftarrow \fG) \eqdef (\fG \to \fF)$,
% \ $\neg \fF \eqdef (\fF \to \bot)$
and
\ $\top \eqdef \sneg \bot$.
We also define the dual of $\bK$ as follows: $\hK \varphi \eqdef \sneg\bK\sneg \varphi$.
We avoid defining $\to$ and $\vee$ in terms of $\wedge$ to avoid the confusion in the following sections where we deal with the intermediate logic of \emph{\mbox{here-and-there}}~\comment{add cite} and where these connectives are not interdefinable.
By $\LEP$ and $\LPP$ we respectively denote the languages containing all epistemic and propositional formulas over~$\at$.

Semantics is given in terms of \emph{epistemic models} and a \emph{updating evaluation} which provides the interpretation for updating objects.
Let us start by introducing epistemic models and its intuition regarding epistemic planning tasks.


\begin{definition}[Epistemic Model]
Given a (possibly infinite) set of propositional symbols~$\at$ and a (possibly infinite) set of possible worlds~$\Worlds$,
a \emph{model} is a
triple
$\cM = \tuple{W,\cK,V}$
where
\begin{itemize}
\item $W \subseteq \Worlds$ is a finite set of worlds,
\item $\cK \subseteq W \times W$ is an accessibility relation on $W$, and
\item $V : W \longrightarrow 2^{\at}$ is a valuation.
\end{itemize}
$D(\cM) = W$
denotes the domain of $M$.
An \emph{epistemic model} is a model where $\cK$ is a equivalent relation. 
An epistemic model where $\cK$ is an universal relation is called a \emph{information cell}.
A \emph{belief model} is a model where \mbox{$\cK = \cK \times \cK'$} with $\cK' = \cK \setminus \set{w_0}$ for some $w_0 \in \cK$.
By $\Models$ we denote the set of all possible epistemic models over~$\at$ and $\Worlds$.\qed
\end{definition}




We adopt an \emph{internal point of view} of epistemic models where the modeller is  the same agent whose knowledge is represented in model.
This contrasts with a \emph{external point of view} where the modeller is assumed to be
an omniscient
and external observer of the epistemic situation who knows which is the actual world~\cite{Aucher10,Fagin95}.
Formally, this translates in the lack of a designated world since the agent considers possible all worlds in model.
A second consequence is that, even for single agent epistemic models, we cannot replace the equivalence relation by a universal one.


% A pair $\emodel{\cM,w}$ consisting of an epistemic model~$\cM$ and a world~\mbox{$w \in D(\cM)$} is called a \emph{pointed (epistemic) model}, while $w$ is refereed as the actual world of~$\emodel{\cM,w}$.
% Intuitively, pointed epistemic models provide a model of the world
% from an external point of view, where the modeller is assumed to be an omniscient
% and external observer of the epistemic situation who knows which is the actual world~\cite{Aucher10}.
% As opposed to this \emph{multi-pointed (epistemic) models} allow representing an internal point of view, where the modeller is one of the agents represented in the
% epistemic model~\cite{Aucher10,Fagin95}.


% Formally, a \emph{multi-pointed (epistemic) model} is a pair $\emodel{\cM,\cW}$ where
% \mbox{$\cW \subseteq D(\cM)$} is a non-empty set of designated worlds.
% Satisfaction a formula~$\varphi$ with respect to \mbox{multi-pointed} epistemic models is defined as follows:
% $\emodel{\cM,\cW} \models \varphi$ iff 
% $\emodel{\cM,w} \models \varphi$ for all $w \in \cW$.
% If $\cW$ is closed under $\cK$, the multi-pointed epistemic model $\emodel{\cM,\cW}$ is  also called a \emph{local (epistemic) state}, in the sense that it may represent the local state of the (planning) agent.
% If $\cW$ is a singleton, $\emodel{\cM,\cW}$ is called a \emph{global (epistemic) state}.
% We will usually write global states pointed as pointed epistemic models, that is, we write 
% $\emodel{\cM,w}$
% instead
% of
% $\emodel{\cM,\set{w}}$.
% Any global state
% $\emodel{\cM,w}$
% has an associated local state
% $\emodel{\cM,\cW}$,
% with $\cW = [w]_\cM$ being
% the set of words accesible from $w$
% and
% defined as 
% \mbox{$ [w]_\cM \eqdef \setm{ w' \in W }{ (w,w') \in \cK }$}.
% In general, we identify a model $\cM$ with the local state $\emodel{\cM,D(\cM)}$ and, in this sense, we write $\cM \models \varphi$ iff $\cM,w\models \varphi$ for all $w \in D(\cM)$.

% As opposed to this \emph{multi-pointed (epistemic) models} allow representing an internal point of view, where the modeller is one of the agents represented in the
% epistemic model~\cite{Aucher10,Fagin95}.
% Formally, a \emph{multi-pointed (epistemic) model} is a pair $\emodel{\cM,\cW}$ where
% \mbox{$\cW \subseteq D(\cM)$} is a non-empty set of designated worlds.
% Satisfaction a formula~$\varphi$ with respect to \mbox{multi-pointed} epistemic models is defined as follows:
% $\emodel{\cM,\cW} \models \varphi$ iff 
% $\emodel{\cM,w} \models \varphi$ for all $w \in \cW$.
% If $\cW$ is closed under $\cK$, the multi-pointed epistemic model $\emodel{\cM,\cW}$ is  also called a \emph{local (epistemic) state}, in the sense that it may represent the local state of the (planning) agent.
% If $\cW$ is a singleton, $\emodel{\cM,\cW}$ is called a \emph{global (epistemic) state}.
% We will usually write global states pointed as pointed epistemic models, that is, we write 
% $\emodel{\cM,w}$
% instead
% of
% $\emodel{\cM,\set{w}}$.
% Any global state
% $\emodel{\cM,w}$
% has an associated local state
% $\emodel{\cM,\cW}$,
% with $\cW = [w]_\cM$ being
% the set of words accesible from $w$
% and
% defined as 
% \mbox{$ [w]_\cM \eqdef \setm{ w' \in W }{ (w,w') \in \cK }$}.
% In general, we identify a model $\cM$ with the local state $\emodel{\cM,D(\cM)}$ and, in this sense, we write $\cM \models \varphi$ iff $\cM,w\models \varphi$ for all $w \in D(\cM)$.
 % \comment{Is it possible to simply this?}

\begin{figure}
\begin{center}
\begin{minipage}{0.4\textwidth}
\begin{center}
\begin{tikzpicture}[align=center,node distance=2.5cm]
\node[point] (w) [label=below:$w_1 : \underline{vl}r\underline{sd}$, label={[label distance=2mm]175:$\cM_0$} ] {};
\node[point] (v) [label=below:$w_2 : \underline{vlrsd}$, right=of w] {};
\path[-] (w) edge (v);
\end{tikzpicture}
\\
(a)
\end{center}
\end{minipage}
\hspace{1cm}
\begin{minipage}{0.4\textwidth}
\begin{center}
\begin{tikzpicture}[align=center,node distance=2.5cm]
\node[point] (w) [label=below:$w_1 : v\underline{l}r\underline{sd}$, label={[label distance=2mm]175:$\cM_1$} ] {};
\node[point] (v) [label=below:$w_2 : v\underline{lrsd}$, right=of w] {};
\path[-] (w) edge (v);
\end{tikzpicture}
\\
(b)
\end{center}
\end{minipage}
\\[20pt]
\begin{minipage}{0.4\textwidth}
\begin{center}
\begin{tikzpicture}[align=center,node distance=2.5cm]
\node[point] (w) [label=below:$w_1 : vlrs\underline{d}$, label={[label distance=2mm]175:$\cM_2$}] {};
\node[point] (v) [label=below:$w_2 : vl\underline{r}s\underline{d}$,right=of w] {};
% \path[-] (w) edge (v);
\end{tikzpicture}
\\
(c)
\end{center}
\end{minipage}
\hspace*{6.7cm}
% \hspace{1cm}
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2.5cm]
% \node[point] (w) [label=below:$w_1 : vlrsd$, label={[label distance=2mm]175:$\cM_3$}] {};
% \node[point] (v) [label=below:$w_2 : vl\underline{r}sd$,right=of w] {};
% % \path[-] (w) edge (v);
% \end{tikzpicture}
% \\
% (d)
% \end{center}
% \end{minipage}
% \\[20pt]
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2.5cm]
% \node[point] (w) [label=below:$w_1 : \underline{v}lrsd$, label={[label distance=2mm]175:$\cM_4$}] {};
% \node[point] (v) [label=below:$w_2 : \underline{v}l\underline{r}sd$,right=of w] {};
% \end{tikzpicture}
% \\
% (e)
% \end{center}
% \end{minipage}
% % \hspace{0.25cm}
% % \begin{minipage}{0.4\textwidth}
% \hspace*{6.65cm}
% \end{minipage}
\end{center}
	\caption{Epistemic models corresponding to the three first states of the execution of the conditional plan~\eqref{eq:pink.conditional.plan}: (a) corresponds to the initial state of Example~\ref{ex:pink}, (b) to the result of executing the action $\move$
	and (c) is the result of flicking the light in the resulting state.
	 % and (d) is the result of performing the actions $\taker$ or $\takel$ depending whether the agents knows that the Pink Panther is on the right or left pedestal.
	 }\label{fig:pink.state0-4}
\end{figure}

\begin{examplecont}{ex:pink}\label{ex:pink.epistemic.models}
Figure~\ref{fig:pink.state0-4} depicts the epistemic models corresponding to the
initial state of Example~\ref{ex:pink} and the two states successively reached from this when executing the plan~$\den{\move ; \, \flick }$.
In other words, we have that $\cM_1$ is the result of executing the action $\move$ in $\cM_0$ and $\cM_2$ is the result of executing the action $\flick$ in $\cM_1$.
We will see later how this intuition is formalised, so let us focus now on the formalisation of each this models.

In particular, Figure~\ref{fig:pink.state0-4}a depicts the epistemic model corresponding to the initial state of Example~\ref{ex:pink},
 that is, the thief is outside the vault ($\underline{v}$), the ligth is off ($\underline{l}$), she cannot see where the Pink Panther is ($\underline{s}$) and she has not the diamond~($\underline{d}$).
The world~$w_1$ corresponds to the possibility that the Pink Panther is on the right pedestal~($r$) while $w_2$ corresponds to the alternative, that is, the diamond is on the left pedestal~($\underline{r}$).
The line between $w_1$ and $w_2$ means that $(w_1,w_2) \in \cK_1$.
Formally, this model corresponds to the triple
\mbox{$\cM_0 = \tuple{W_0,\cK_0,V_0}$}
with two worlds $W_0=\set{w_1,w_2}$, a universal accessibility relation $\cK_0 = W_0 \times W_0 = \set{ (w_1,w_2), (w_2, w_1) }$
and with a valuation $V_0$ satisfying $V_0(w_1) = \set{r}$ and $V_0(w_2) = \emptyset$.
The epistemic model $\cM_1$ in Figure~\ref{fig:pink.state0-4}b is very similar with the only exception that now the thief is in the vault ($v$).
That is,
\mbox{$\cM_1 = \tuple{W_0,\cK_0,V_1}$}
with $V_1$ satisfying $V_1(w_1) = \set{v,r}$ and $V_0(w_2) = \set{v}$.

On the other hand, 
Figure~\ref{fig:pink.state0-4}c shows the epistemic model represeting the result of performing the action $\flick$ in $\cM_1$, with worlds $w_1$ and $w_2$ representing the results of performing these two actions on worlds $w_1$ and $w_2$ of~$\cM_1$, respectively.
Formally, we have that
$\cM_2 = \tuple{W_0,\cK_2,V_2}$
with
% $W_2=\set{w_1,w_2}$, 
$\cK_2 = \emptyset$
and with $V_2$ satisfying $V_2(w_1) = \set{v,l,r,s}$ and $V_2(w_2) = \set{v,l,s}$.
\qed
\end{examplecont}


Note that in the above example, the relation of accessibility of $\cM_2$ is not a universal relation.
As mentioned above, this reflects the internal perspective of the agent.
To make this more precise, we introduce two conceps of indistinguishableness.
% \begin{definition}[Run-time and plan-time indistinguishableness]
Given an epistemic model
\mbox{$\cM = \tuple{W,\cK,V}$}, any two worlds
\mbox{$w,w' \in W$} are called \emph{run-time indistinguishable} iff
\mbox{$(w,w') \in \cK$}.
Any two worlds
\mbox{$w,w' \in W$}
are called \emph{\mbox{plan-time} indistinguishable} iff \mbox{$(w,w')\notin \cK$}.
% Given an epistemic model~$\cM$, we say that two worlds $w_1,w_2 \in D(\cM)$ are \emph{run-time indistinguishable} (resp. \emph{\mbox{plan-time} indistinguishable}) iff they are  run-time indistinguishable (resp. \mbox{plan-time} indistinguishable) with respect to the local state $\emodel{\cM,D(\cM)}$.
% \qed
% \end{definition}

% the agent knows that she can distinguish between worlds $w_1$ and $w_2$



 % \comment{No definition} 







\begin{examplecont}{ex:pink.epistemic.models}\label{ex:pink.indistinguishableness}
Continuing with our running example, 
worlds $w_1$ and $w_2$ are plan-time indistinguishable with respect to the model~$\cM_2$ because $(w_1,w_2) \notin \cK_2$, that is,  $w_1$ and $w_2$ are disconnected in Figure~\ref{fig:pink.trans0-1}b.
This means that, though the agent does not know at planning time which of the two possibilities represented by worlds $w_1$ and $w_2$ will correspond to the actual world, she will discover it when performing the sequence of actions and, thus, she will be able to act in consequence.
In this particular case, this means that when planning she is not able to know whether the Pink Panther is on the right or left pedestal, but that when performing the actions of the plan to reach that state, she will eventually learn in which pedestal it is.
As a result, at that point, she will be able to make a decision whether she should perform the $\taker$ or $\takel$ action.

In contrast, worlds~$w_1$ and~$w_2$ are run-time indistinguishable with respect to the model~$\cM_1$ because
$(w_1,w_2) \notin \cK_1$.
This means that the agent is not able to distinguish between the two possibilities represented by worlds~$w_1$ and~$w_2$, neither when she is computing the plan nor later on when she would be executing the actions of the plan.
In consequence, even when executing the plan, the agent cannot make any decision based on the actual world.
\qed
\end{examplecont}


% Consider a local state $s = \emodel{\cM,\cW}$ containing only $w$ and $v$, and that these are plan-time indistinguishable. This means, that while the agent is planning, it does not know whether the actual world is $w$ or $v$. However, when the plan is being executed and the agent actually achieves the state of the world represented by $s$, it will know which of $w$ and $v$ is the actual world.
% In other words, the agent knows, that while it does not yet know the actual world, it will come to know this once the plan is being carried out. If $w$ and $v$ are run-time indistinguishable, then the agent is unable to distinguish them, both while planning and when carrying out the plan.


%  \comment{
% Note that the fact that worlds $w_1$ and $w_2$ are connected in $\cM_1$ means that they are run-time indistinguishable, that is, the agent does not know at planning time nor she will know when performing the plan which of the two possible worlds corresponds the actual world.
% On the other hand, fact that worlds $w_1$ and $w_2$ are disconnected in $\cM_2$ means they are only plan-time indistinguishable, that is, though the agent does not know at planning time which of the two possible worlds will be the actual world, she will discover it when performing this sequence of actions.}

%  \comment{
% In general, we identify a model $\cM=\tuple{W,\cK,V}$ with the local state $\emodel{\cM,W}$ so that all worlds in $W$ is considered plan-time indistinguishable while each pair of worlds $(w,w') \in \cK$ are considered runt-time indistinguishable.
% In this sense, we write $\cM \models \varphi$ iff $\cM,w\models \varphi$ for all $w \in W$.}
% Figure~\ref{fig:pink.state0-4} shows the epistemic models corresponding the conditional plan~\eqref{eq:pink.conditional.plan}.
% In particular, Figure~\ref{fig:pink.state0-4}a shows the epistemic model corresponding to the initial state of Example~\ref{ex:pink},
%  that is, the thief is outside the vault ($\underline{v}$), the ligth is off ($\underline{l}$), she cannot see where the Pink Panther is ($\underline{s}$) and she has not the diamond~($\underline{d}$).
% The world~$w_1$ corresponds to the possibility that the Pink Panther is on the right pedestal ($r$) while $w_2$ corresponds to the alternative, that is, the diamond is on the left pedestal ($\underline{r}$).
% The line between $w_1$ and $w_2$ means that $(w_1,w_2) \in \cK_1$.
% Formally, this corresponds to the epistemic model 
% $\cM_0 = \tuple{W_0,\cK_0,V_0}$
% with $W_0=\set{w_1,w_2}$, $\cK_0 = W_0 \times W_0 = \set{ (w_1,w_2), (w_2, w_1) }$
% and with $V_1$ satisfying $V_0(w_1) = \set{r}$ and $V_0(w_2) = \emptyset$.
% On the other hand, 
% Figure~\ref{fig:pink.state0-4}c shows the epistemic model represeting the result of performing the action $\move$ following by the action $\flick$, with worlds $w_1$ and $w_2$ representing the results of performing this actions on worlds $w_1$ and $w_2$ or $\cM_0$, respectively.
% Formally, we have that
% $\cM_2 = \tuple{W_2,\cK_2,V_2}$
% with $W_2=\set{w_1,w_2}$, $\cK_2 = \emptyset$
% and with $V_3$ satisfying $V_2(w_1) = \set{vlrs}$ and $V_2(w_2) = \set{vls}$.
% Note that the fact that worlds $w_1$ and $w_2$ are connected in $\cM_1$ means that they are run-time indistinguishable, that is, the agent does not know at planning time nor she will know when performing the plan which of the two possible worlds corresponds the actual world.
% On the other hand, fact that worlds $w_1$ and $w_2$ are disconnected in $\cM_2$ means they are only plan-time indistinguishable, that is, though the agent does not know at planning time which of the two possible worlds will be the actual world, she will discover it when performing this sequence of actions.






As mentioned above, satisfaction of formulas is defined with respect to an
\emph{updating evaluation}.
Let us now formalise this concept.

\begin{definition}[Updating evaluation]
Given a set of models $\Models$ over set of worlds $\Worlds$ and a set of updating objects $\uobj$,
an \emph{updating evaluation}
is a pair $\tuple{\otimes,\cR}$
of functions
\mbox{$\otimes : \Models \times \uobj \longrightarrow \Models$},
and
\mbox{$\cR : \Models \times \uobj \longrightarrow 2^{\Worlds \times \Worlds}$}
% and
% \mbox{$\pre : \uobj \longrightarrow 2^{\Models \times \Worlds}$}
satisfying
$\cR(\cM,o) \subseteq D(W) \times D(\otimes(\cM, o))$.\qed
\end{definition}

We will usually write $\otimes$ in infix notation and assume that it is left associative 
so that $\cM \otimes o$ stands for $\otimes(\cM,o)$
and
$\cM \otimes o_1 \otimes o_2$ stands for $(\cM \otimes o_1) \otimes o_2$.
We will also write $\cR_{\cM,o}$ instead of $\cR(\cM,o)$ so that
$\cR_{\cM,o} \subseteq D(W) \times D(\cM\otimes o)$
is a relation between the worlds of $\cM$ and $\cM\otimes o$.





\begin{definition}[Satisfaction]
\label{def:del.sat}
Let
\mbox{$\tuple{\otimes,\cR}$}
be an updating evaluation.
Then, given an epistemic model~\mbox{$\cM = \tuple{W,\cK,V}$},
satisfaction of formulas is given by the following recursive definition:
\begin{itemize}
\item $\cM, w \not\models \bot$,
\item $\cM, w \models p$ iff $p \in V(w)$,
\item $\cM, w \models \varphi_1 \wedge \varphi_2$ iff $\cM, w \models \varphi_1$ and $\cM, w \models \varphi_2$,
\item $\cM, w \models \varphi_1 \vee \varphi_2$ iff $\cM, w \models \varphi_1$ or $\cM, w \models \varphi_2$,

\item $\cM, w \models \varphi_1 \to \varphi_2$ iff $\cM, w \not\models \varphi_1$ or $\cM, w \models \varphi_2$,

\item $\cM, w \models \sneg \varphi$ iff $\cM, w \not\models \varphi$,

\item $\cM, w \models \bK \varphi$ iff $\cM, w' \models \varphi$ for all $w'$ with $(w,w') \in \cK$, and

\item $\cM, w \models [o] \varphi$ iff $\cM \otimes o, w' \models \varphi$ for all $w'$ with $(w,w') \in \erelation{\cM}{o}$.
% and $\tuple{\cM,w} \in \pre(o)$.
\qed
\end{itemize}

\end{definition}

As usual, we write
\mbox{$\cM \models \varphi$} iff
\mbox{$\cM,w\models\varphi$} for every world
\mbox{$w \in W$}.
Furthermore, given a theory
$\Gamma$, we write
\mbox{$\cM \models \Gamma$} iff
\mbox{$\cM \models \varphi$} for every formula
\mbox{$\varphi \in \Gamma$} and
\mbox{$\Gamma \models \psi$} iff every epistemic model
\mbox{$\cM \in \Models$} satisfies
\mbox{$\cM \models \psi$} whenever
\mbox{$\cM \models \Gamma$} holds.

It is easy to see that, if we restrict ourselves to formulas without the dynamic operator $[\cdot]\cdot$, the semantics of formulas corresponds to the standard modal logic S5 (see~\cite{halpern1986reasoning} for instance).
Let us now see how this definitions apply to the case in which updating objects are event models~\cite{BatlagMS98}.
The following is an adaptation of the definition from~\cite{AndersenBJ12}.

\begin{definition}[Event Model]
An \emph{event model} over $\at$ and $\Worlds$ is a quadruple $\cE = \tuple{E,\cK,\pre,\post}$
where
\begin{itemize}
\item $E \subseteq \Worlds$ is a finite set of worlds called \emph{events},
\item $\pre : E \longrightarrow \LEP$ assigns to each event a precondition, and
\item $\post : E \longrightarrow (\at \longrightarrow \LEP)$ assigns to each event a postcondition.
\end{itemize}
By $D(\cE) = E$ we denote the domain of $\cE$.
A pair $\tuple{\cE,e}$ with $e \in E$ is called a \emph{pointed event model}.\qed
\end{definition}


\begin{definition}[Event updating evaluation]
Let
\mbox{$\cM = \tuple{W,\cK,V}$}
e an epistemic model and
\mbox{$\cE = \tuple{E,\cK,\pre,\post}$}
be an event model, both over $\at$ and~$\Worlds$.
The \emph{product update} of $\cM$ with $\cE$ is the epistemic model denoted
$\cM \otimes \cE \eqdef \tuple{W',\cK'',V'}$ with
\begin{itemize}
\item $W' = \setm{ (w,e) \in W \times E}{ \cM,w \models \pre(e)} \subseteq \Worlds$ is a set of worlds,
\item $\cK'' = \setm{((w_1,e_1),(w_2,e_2)) \in W' \times W' }{ (w_1,w_2) \in \cK \text{ and } (e_1,e_2) \in \cK' }$,
\item $V'((w,e)) = \setm{p \in \at}{ \cM,w \models\post(e)(p) }$ for every $(w,e) \in W'$,
\end{itemize}
% We also define
% $\cR(\cM,\cE) = \setm{(w,(w,e)) \in W \times W'}{ e \in E }$.

Given a pointed event model $\tuple{\cE,e}$,
the \emph{event updating evaluation} is a triple $\tuple{\otimes,\cR,\pre}$
with
\begin{itemize}
\item $\cM \otimes \tuple{\cE,e} \eqdef \cM \otimes \cE$
\item $\cR(\cM,\tuple{\cE,e}) \eqdef \setm{(w,(w,e)) \in W \times W' }{ \cM,w \models \pre(e) }$.\qed
% \item $\pre(\tuple{\cE,e}) \eqdef \setm{ \tuple{\cM,w} }{ \cM,w \models \pre(e) }$.\qed
\end{itemize}
\end{definition}

In the sake of clarity,
we will usually write $[\cE,e] \varphi$ instead of $[\tuple{\cE,e}] \varphi$.
We will also use the following shorthands
\begin{gather*}
[\cE] \varphi \ \eqdef \ \bigwedge_{e \in D(\cE)} [\cE,e] \varphi
\hspace{2cm}
\tuple{\cE} \varphi \ \eqdef \ \sneg\,[\cE]\sneg\varphi
\end{gather*}

The following result shows that, indeed, the semantics described above coincides with the semantics from~\cite{AndersenBJ12} for the case of event models.

\begin{proposition}
Let $\cM$ be an epistemic model, $w \in D(\cM)$ be a world in $\cM$,
$\tuple{\cE,e}$ be pointed event model and $\varphi \in \LEP$ be a formula.Then,
\begin{itemize}
\item $\cM,w \models [\cE,e] \varphi$ iff $\cM,w \models \pre(e)$ implies $\cM \otimes \cE, (w,e) \models \varphi$,

\item $\cM,w \models [\cE] \varphi$ iff $\cM \otimes \cE, (w,e) \models \varphi$ for every $e \in D(\cE)$ such that $\cM,w \models \pre(e)$,

\item $\cM,w \models \tuple{\cE} \varphi$ iff $\cM,w \models \pre(e)$ and $\cM \otimes \cE, (w,e) \models \varphi$ for some $e \in D(\cE)$.
\end{itemize}
\end{proposition}

\begin{proof}
By definition, we have $\cM,w \models [\cE,e]$
\\iff
$\cM \otimes \tuple{\cE,e}, w' \models \varphi$ for all $w'$ with $(w,w') \in \erelation{\cM}{\tuple{\cE,e}}$
\\iff
$\cM \otimes \cE, w' \models \varphi$ for all $w'$ with $(w,w') \in \erelation{\cM}{\tuple{\cE,e}}$.
\\
Note now that, by definition, we have either
$\erelation{\cM}{\tuple{\cE,e}} \cap (\set{w} \times D(\cM \otimes \cE)) = \set{(w,(w,e))}$
or $\erelation{\cM}{\tuple{\cE,e}} \cap (\set{w} \times D(\cM \otimes \cE)) = \emptyset$.
Hence, the above holds
\\iff
$\cM \otimes \cE, (w,e) \models \varphi$ or $\erelation{\cM}{\tuple{\cE,e}} \cap (\set{w} \times D(\cM \otimes \cE)) = \emptyset$,
\\iff
$\cM \otimes \cE, (w,e) \models \varphi$ or $\cM,w \not\models \pre(e)$
\\iff
$\cM,w \models \pre(e)$ implies $\cM \otimes \cE, (w,e) \models \varphi$.
\\[10pt]
The second statement follow directly from its definitions.
For the third, we have
$\cM,w \models \tuple{\cE} \varphi$
iff
$\cM,w \models \sneg\,[\cE] \sneg \varphi$
iff
$\cM,w \not\models [\cE] \sneg \varphi$
\\iff
$\cM,w \models \pre(e)$ does not imply $\cM \otimes \cE, (w,e) \models \sneg\varphi$ for some $e \in D(\cE)$
\\iff
$\cM,w \models \pre(e)$ and $\cM \otimes \cE, (w,e) \not\models \sneg\varphi$ for some $e \in D(\cE)$
\\iff
$\cM,w \models \pre(e)$ and $\cM \otimes \cE, (w,e) \models \varphi$ for some $e \in D(\cE)$.
\end{proof}










%  \comment{
% Given an epistemic model~$\cM = \tuple{W,\cK,V}$, satisfaction of epistemic formulas is given by the following recursive definition:
% \begin{itemize}
% \item $\cM, w \not\models \bot$,
% \item $\cM, w \models p$ iff $p \in V(w)$,
% \item $\cM, w \models \varphi_1 \wedge \varphi_2$ iff $\cM, w \models \varphi_1$ and $\cM, w \models \varphi_2$,
% \item $\cM, w \models \varphi_1 \vee \varphi_2$ iff $\cM, w \models \varphi_1$ or $\cM, w \models \varphi_2$,

% \item $\cM, w \models \varphi_1 \to \varphi_2$ iff $\cM, w \not\models \varphi_1$ or $\cM, w \models \varphi_2$,

% \item $\cM, w \models \sneg \varphi$ iff $\cM, w \not\models \varphi$,

% \item $\cM, w \models \bK \varphi$ iff $\cM, w' \models \varphi$ for all $w'$ with $(w,w') \in \cK$
% \end{itemize}
% }






% The following result shows that every information cell can be characterised by some epistemic formula.

%  \comment{move this?}



%  \comment{Do we need the following? 
% Every information cell can be represented (up to bisimilarity) by some epistemic formula as follows.

% \begin{definition}\label{def:char.epistemic}
% Given some information cell $\cM = \tuple{W,\cK,V}$,
% its \emph{characteristic epistemic formula} is 
% $\varphi_\cM \eqdef \bK (\bigwedge_{w \in W} \tK \varphi_\cM^w) \wedge \bigvee_{w \in W}  \bK \varphi_\cM^w)$
% % \begin{gather*}
% % \varphi_\cM \quad \eqdef \quad \Big(\bigwedge_{w \in W} \bM \varphi_w \Big) \wedge \Big(\bK\bigvee_{w \in W}  \varphi_w \Big)
% % \end{gather*}
% where $\varphi_\cM^w$ is defined as follows:
% \begin{gather*}
% \varphi_\cM^w \quad \eqdef \quad \Big(\bigwedge_{p \in V(w)} p \Big) \wedge \Big( \bigwedge_{p \in \overline{V(w)}} \sneg p\Big)
% \end{gather*}
% \end{definition}

% \begin{lemma}[Lemma~1 in \cite{AndersenBJ12}]\label{lem:char.epistemic}
% Let $\cM_1$ be an information cell.
% Then for all epistemic models $\cM_2 = \tuple{W_2,\cK_2,V_2}$ and all $w_2 \in W_2$ we have that 
% \mbox{$\cM_2, w_2 \models \varphi_\cM$} iff there exists some $w_1 \in D(\cM_1)$
% such that $(\cM_1,w_1)$ and $(\cM_2,w_2)$ are bisimilar.
% \end{lemma}

% }


\section{Founded Autoepistemic Equilibrium Logic with Strong Negation}

In this section we review the definition of Founded Autoepistemic Equilibrium Logic (FAEL) from~\comment{add cite} extended 
with a \emph{strong negation}~$``\!\sneg\,$'' connective~\cite{nelson1949,GelfondL91,Pearce96}.
By abuse of notation we use the symbol~``$\sneg\,$'' for both classical negation and strong negation depending on the context.
The motivation for this abuse is that we will use strong negation in FAEL to capture the same intuitive meaning that classical negation has in epistemic models.
In fact, we will show how any information cell can be represented as an formula in \FAEEL in which strong negation represents the false atoms in the model.
\emph{Autoepistemic formulas} are defined according to the following grammar:
\[
\fF ::= \bot \mid p \mid \sneg p \mid \fF_1 \wedge \fF_2 \mid \fF_1 \vee \fF_2 \mid \fF_1 \to \fF_2 \mid \bL \varphi
% \mid \bM \varphi
% \qquad\text{ for any atom } a \in \at. 
\]
where \mbox{$p \in \at$} is a proposition.
A \emph{literal}~$L$ is either a proposition $p \in \at$ or a proposition preceded by strong negation~$\sneg p$.
By $\lit \eqdef \at \cup \sneg\at$ we denote the set of all literals over $\at$
where $\sneg S \eqdef \setm{ \sneg p }{ p \in S }$ is the set of all negated literals corresponding to any set of propositions $S \subseteq \at$.
Intuitively, $\bL\varphi$ is read as ``is reasonable (for the planning agent) to believe~$\varphi$.''
% while $\bM\varphi$ is read as `is reasonable (for the planning agent) to believe that~$\varphi$ is possible.''
Weak or intuitionistic negation is defined as usual: $\neg\varphi \eqdef \varphi \to \bot$.
The knowledge modality is defined as:
$\bK \varphi = \varphi \wedge \bL \varphi$.
% and
% $\hM \varphi = \varphi \vee \bM \varphi$.
We also assume all above abbreviations, that is,
\mbox{$(\fF \leftarrow \fG) \eqdef (\fG \to \fF)$},
\
\mbox{$\fF \leftrightarrow \fG \eqdef (\fF \to \fG) \wedge (\fG \to \fF)$},
% \ $\neg \fF \eqdef (\fF \to \bot)$
and
\ $\top \eqdef \bot\to\bot$.
% and
% \ $\hK \varphi \eqdef \sneg\bK\sneg\varphi$
% We also define the dual of $\bK$ as follows: $\hK \varphi \eqdef \sneg\bK\sneg \varphi$.
An \emph{autoepistemic theory}~$\Gamma$ is a set of autoepistemic formulas as defined above.
When a theory is a singleton, we will usually write just $\varphi$ instead of~$\set{\varphi}$.
% Besides, we assume that in addition to the formulas explicitly mentioned in each theory, every theory implicitly contains a formula of the form:
% \begin{gather}
% \bot \leftarrow \neg\!\bL(p \wedge \sneg p)
% 	\label{eq:sneg}
% \end{gather}
% for every proposition~$p \in \at$,
% stating that the agent cannot believe in contradictions.


\begin{definition}[HT-Model]
Given a set of propositional symbols~$\at$,
an \emph{\htmodel} is a
quadruple
\mbox{$\cM = \tuple{W,\cK,V^h,V^t}$}
where
\begin{itemize}
\item $W$ is a set of worlds,
\item $\cK \subseteq W \times W$ is an accessibility relation on $W$, and
\item $V^x : W \longrightarrow 2^{\lit}$ is a valuation with $x \in \set{h,t}$ 
such that \mbox{$V^h(w) \subseteq V^t(w)$} 
% and either $p \notin V^t(w)$ or $\sneg p \notin V^t(w)$
for all $w \in W$.
\end{itemize}
$D(\cM) = W$
denotes the domain of $M$.
% An \emph{epistemic \htmodel} is a \htmodel where $\cK$ is a equivalent relation and 
A \emph{belief \htmodel} is an \htmodel where $\cK = \cK \times \cK'$ with $\cK' = \cK \setminus \set{w_0}$ for some \emph{distinguish world} $w_0 \in \cK$.
% An epistemic model where $\cK$ is an universal relation is called a \emph{\htinformation cell}.
\qed
\end{definition}
A \htmodel $\cM = \tuple{W,\cK,V^h,V^t}$ is called \emph{total}
iff $V^h = V^t$.
Furthermore, by $\cM^t \eqdef \tuple{W,\cK,V^t,V^t}$ we denote the total model corresponding to~$\cM$.
Satisfaction of epistemic formulas is then given by the following recursive definition:
\begin{itemize}
\item $\cM, w \not\models \bot$,
\item $\cM, w \models L$ iff $L \in V^h(w)$,
\item $\cM, w \models \varphi_1 \wedge \varphi_2$ iff $\cM, w \models \varphi_1$ and $\cM, w \models \varphi_2$,
\item $\cM, w \models \varphi_1 \vee \varphi_2$ iff $\cM, w \models \varphi_1$ or $\cM, w \models \varphi_2$,

\item $\cM, w \models \varphi_1 \to \varphi_2$ iff
both $\cM, w \not\models \varphi_1$ or $\cM, w \models \varphi_2$
and\\
\hspace*{4.6cm}
$\cM^t, w \not\models \varphi_1$ or $\cM^t, w \models \varphi_2$,

% \item $\cM, w \models \sneg \varphi$ iff $\cM, w \not\models \varphi$,

\item $\cM, w \models \bK \varphi$ iff $\cM, w' \models \varphi$ for all $w'$ with $(w,w') \in \cK$
\end{itemize}
As usual, we say that $\cM$ is a \emph{\htmodel} of some theory~$\Gamma$, in symbols \mbox{$\cM \models \Gamma$}, iff
\mbox{$\cM,w\models \varphi$} for every world~$w \in D(\cM)$ and every formula~$\varphi \in \Gamma$.



\begin{definition}[Bisimulation for HT-models]\label{def:int.prec}
Let
\mbox{$\cM_1 = \tuple{W_1,\cK_1,V_1^h,V_1^t}$}
and
\mbox{$\cM_2 = \tuple{W_2,\cK_2,V_2^h,V_2^t}$}
be two \htmodels.
Given a relation $Z \subseteq W_1\times W_2$,
we write $\cM_1 \preceq^Z \cM_2$ iff
\begin{itemize}
\item every $(w_1,w_2) \in Z$ satisfies $V^t(w_1) = V^t(w_2)$ and  $V^h(w_1) \subseteq V^h(w_2)$,

\item for every $(w_1,w_1') \in \cK_2$, there is $(w_2,w_2') \in \cK_2$ such that $(w_1',w_2') \in Z$,

\item for every $(w_2,w_2') \in \cK_2$, there is $(w_1,w_1') \in \cK_2$ s.t.
\mbox{$(w_1',w_2') \in Z$}.
\end{itemize}
We write $\cM_1 \preceq \cM_2$ iff there is a total relation $Z$ s.t. $\cM_1 \preceq^Z \cM_2$.
We also say that $\cM_1$ and $\cM_2$ are \emph{bisimilar} iff, in symbols $\cM_1 \approx \cM_2$,
there is a total relation $Z$ s.t $\cM_1 \preceq^Z \cM_2$ and $\cM_2 \preceq^Z \cM_1$.
As usual, we write
$\cM_1 \prec \cM_2$ iff $\cM_1 \preceq \cM_2$ and $\cM_1 \not\approx \cM_2$.\qed
\end{definition}
% Given two \htmodels
% \mbox{$\cM_1 = \tuple{W_1,\cK_1,V_1^h,V_1^t}$}
% and
% \mbox{$\cM_2 = \tuple{W_2,\cK_2,V_2^h,V_2^t}$}
% and a relation
% \mbox{$Z \subseteq W_1 \times W_2$},
% we write
% $\cM_1 \preceq^x_Z \cM_2$ with $x \in \set{h,t}$
% iff, for every $(w_1,w_2) \in Z$, the following two condition hold:
% \begin{itemize}
% \item $V^x(w_1) \subseteq V^x(w_2)$, and
% \item for every $(w_1,w_1') \in \cK_2$, there is $(w_2,w_2') \in \cK_2$ such that $(w_1',w_2') \in Z$.
% \item for every $(w_2,w_2') \in \cK_2$, there is $(w_1,w_1') \in \cK_2$ such that $(w_1',w_2') \in Z$.
% \end{itemize}
% We write $\cM_1 \approx^x_Z \cM_2$ iff
% $\cM_1 \preceq^x_Z \cM_2$
% and
% $\cM_1 \succeq^x_Z \cM_2$.
% We say that two models $\cM_1$ and $\cM_2$ are \emph{there-bisimilar} iff there is a total relation $Z$ such that $\cM_1 \approx^t_Z \cM_2$.
% \begin{definition}\label{def:int.prec}
% We define the partial order $\cM_1 \preceq \cM_2$ for \htmodels
% when there is a total relation $Z$ such that
% $\cM_1 \approx_Z^t \cM_2$ and $\cM_1 \preceq_Z^h \cM_2$.\qed
% \end{definition}
% As usual, we write
% % $\cM_1 \succeq \cM_2$
% % iff
% % $\cM_2 \preceq \cM_1$.
% % We say that two models $\cM_1$ and $\cM_2$ are \emph{bisimilar} iff $\cM_1 \preceq \cM_2$ and $\cM_1 \succeq \cM_2$.
% % We also write
% $\cM_1 \prec \cM_2$ iff $\cM_1 \preceq \cM_2$ and $\cM_1 \not\approx \cM_2$.


\begin{definition}[Equilibrium model]
A total belief \htmodel $\cM$ of some theory~$\Gamma$ is said to be a \emph{equilibrium model} of ~$\Gamma$ iff there is no other belief \htmodel~$\cM'$ of $\Gamma$ such that $\cM' \prec \cM$.\qed
\end{definition}





Given some information cell $\cM = \tuple{W,\cK,V}$ and some set of literals
\mbox{$I\subseteq \lit$},
by $\cM + I$ we denote the belief \htmodel
$\cM' = \tuple{W',\cK',V'}$
where
\mbox{$W' = \set{w_0} \cup W$} with $w_0 \notin W$, \, $\cK' = W' \times W$ and
$V' : W' \longrightarrow 2^{\lit}$
satisfies $V'(w) = V(w)$ for all $w \in W$ and $V'(w_0) = I$.

\begin{definition}[World view]
Given a set of propositions~$\at$,
a information cell $\cM = \tuple{W,\cK,V}$ over $\lit$ is called a \emph{world view} of some theory~$\Gamma$ iff the following two condition hold:
\begin{itemize}
\item $\cM + V(w)$ is an equilibrium model of $\Gamma$ for all world $w \in W$,

\item $\cM + I$ is not an equilibrium model of $\Gamma$ for all set of literals $I \subseteq \lit$ satisfying $I \neq V(w)$ for all $w \in W$, and

\item either $p \notin V^t(w)$ or $\sneg p \notin V^t(w)$ for all $p \in \at$ and $w \in W$.
\end{itemize}
We say that a theory~$\Gamma$ is \emph{consistent} iff it has some world view.\qed
\end{definition}




\begin{examplecont}{ex:pink.indistinguishableness}\label{ex:pink.formula}
For instance, the formula
\begin{gather}
\varphi_0 = \sneg v \wedge \sneg l \wedge (r \vee \sneg r) \wedge \sneg s \wedge \sneg d
	\label{eq:formula.state0}
\end{gather}
has a unique world view that is depicted in Figure~\ref{fig:pink.state0.auto}.
 \comment{calculation}\qed
\end{examplecont}

==> motivation.tex <==
%!TEX root = main.tex

% \documentclass{svproc}

% \usepackage[utf8]{inputenc}
% \usepackage{amsmath,amssymb}
% \usepackage{tikz}
% \usetikzlibrary{positioning,arrows,calc}
% \tikzset{
% modal/.style={>=stealth’,shorten >=1pt,shorten <=1pt,auto,node distance=1.5cm,
% semithick},
% world/.style={circle,draw,minimum size=0.5cm,fill=gray!15},
% point/.style={circle,draw,inner sep=0.5mm,fill=black},
% reflexive above/.style={->,loop,looseness=7,in=120,out=60},
% reflexive below/.style={->,loop,looseness=7,in=240,out=300},
% reflexive left/.style={->,loop,looseness=7,in=150,out=210},
% reflexive right/.style={->,loop,looseness=7,in=30,out=330}
% }
% \usepackage{microtype}
% \usepackage{listings}
% \lstset{numbers=left,numberblanklines=false,basicstyle=\ttfamily}
% \usepackage{bm}
% \usepackage{multirow}
% \usepackage{textcomp}
% \usepackage{url}
% \usepackage{IEEEtrantools}
% \usepackage{enumitem}
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{array}
% \usepackage{stmaryrd}
% \usepackage{graphicx}
% \input{macro}
% \input{outline}
% \usepackage[comments=on,changes=on]{krudces}
% \bibliographystyle{splncs03}

% \title{Single-agent Conditional Epistemic Planning in Dynamic Epistemic Answer Set Programming}
% \author{
% Pedro Cabalar \inst{1} \and
% Jorge Fandinno \inst{2} \and 
% Luis Fari{\~n}as \inst{2}
% }
% \institute{University of Corunna, Spain\\
% \email{cabalar@udc.es}
% \and University of Toulouse IRIT, CNRS, France\\
% \email{\{jorge.fandinno,farinas\}@irit.fr}
% }

% \begin{document}





% \maketitle





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Motivation}\label{sec:motivation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To further motivate our ideas, let us start by introducing the following example from~\cite{AndersenBJ12}, which will constitute our running example through the~paper.
% (Example~\ref{ex:pink}).

\begin{example}
% \label{ex:pink}
After following carefully laid plans, a thief has almost made it to
her target: the vault containing the invaluable Pink Panther diamond.
Standing outside the vault, she now deliberates on how to get her hands on the
diamond.
She \emph{knows} the light inside the vault is off, and that \emph{the Pink
Panther is on either the right or left pedestal inside.}
Obviously, the
diamond cannot be on both the right and left pedestal, but nonetheless the
agent may be uncertain about its location.
Note that the thief is perfectly capable of moving in the darkness and take whatever is on top any of the pedestals, but she is not able to know whether the diamond has been taken or not.
It is assumed that there are four possible actions: $\move$, $\flick$, $\takel$ and $\taker$.
The action $\move$ changes the location of the thief from ouside the vault~($\sneg v$) to inside the vault~($v$) and vice-versa.
The action $\flick$ turns on the light ($l$).
Furthermore, \emph{if the thief is in the vault ($v$) and the light is on ($l$), the thief can see~($s$) where the Pink Panther is.}
Finally, actions $\takel$ and $\taker$ respectively take the diamond ($d$) from the left ($\sneg r$) or right ($r$) pedestal
if the diamond is the intended pedestal and have no effect otherwise.
\qed
\end{example}


A first plan to be considered by the thief may consist in the following sequence of actions
$\pi_{c} = \den{\move;\, \takel;\, \taker;\, \move}$.
In other words, the thief moves inside the vault and then takes all items that are in the left and right pedestal, in this order, and finally she moves outside of the vault.
This way, she may be sure that she has taken the diamond despite whether it is in the right or left pedestal.
This is what is known as a \emph{conformant plan}, that is, a sequence of actions that succeed in achieving the goal no matter
which of the allowed states the world is actually in~\cite{SmithW98}.
On the other hand, if we consider that  expending the time for taking objects from the two pedestals is not desirable, we can opt for \emph{flicking} the light after entering the vault.
This way, the agent will discover in which pedestal is the Pick Panther and, thus, take it directly from its location.
This is what is know as a \emph{conditional plan}, that is,
a sequence of actions which are conditioned on observations made prior to their execution~\cite{peot1992conditional}.
For instance, in our running example, this conditional plan can be writing as
\begin{gather}
\den{\move ; \, \flick ; \, \iif \bK r \tthen \taker \eelse \takel ;\, \move}
	\label{eq:pink.conditional.plan}
\end{gather}
where $\bK r$ stands for ``at the moment of carrying the plan on, the (planning) agent knows that $r$ holds.''
According to this knowledge, she will make the decision to take what is in the right or the left pedestal.

As mentioned in the introduction, ASP is a knowledge representation formalism that allows \comment{...}
For instance, the following simplification of Example~\ref{ex:pink}
where the whole initial state is know is easily representable in ASP.


\begin{examplecont}{ex:pink}\label{ex:pink.simple}
Consider now the case where the thief is outside the vault ($\sneg v$) and already \emph{knows the Pink Panther is inside the vault on the right ($r$) pedestal}.\qed
\end{examplecont}


Since in this example the value of all fluents at the initial situation are known, we can ignore the sensing effect of being in the vault with the light turned on.
In such case, we can represent the domain of these examples as the following temporal logic program~\cite{CabalarKSS18}:
\begin{IEEEeqnarray}{c C l}
v &\leftarrow& \move \wedge \previous\sneg v
	\label{eq:pink.1}
\\
\sneg v &\leftarrow& \move \wedge \previous v
\\
l &\leftarrow& \flick
\\
d &\leftarrow& \takel \wedge \previous v \wedge \previous \sneg  r
\\
d &\leftarrow& \taker \wedge \previous v \wedge \previous r
	\label{eq:pink.5}
\\
s &\leftarrow& v \wedge l
\end{IEEEeqnarray}
where $\previous \varphi$ intuitivelly means that the formula~$\varphi$ was true in the previous state.
As usual, we distinguish two kinds of propositions respectivelly called \emph{actions} and \emph{fluents} \comment{add cite}.
In our running example,
we have a set of actions
\mbox{$\cA = \set{\move,\flick,\taker,\takel}$}
and of fluents
\mbox{$\cF = \set{v,l,d,s}$}.
We further divide the set of fluents in \emph{inertial} 
$\cF^\cI = \set{v,l,d}$ and \emph{non-inertial} fluents
$\cF^\cN = \set{s}$.
The state that the value of \emph{inertial fluents}
remains the same unless stated otherwise.
This is captured by adding the following \emph{inertial axioms}:
\begin{IEEEeqnarray}{c C l}
f &\leftarrow& \previous f \wedge \neg\!\sneg f
	\label{eq:pink.6}
\\
\sneg f &\leftarrow& \previous \sneg f \wedge \neg f
	\label{eq:pink.7}
\end{IEEEeqnarray}
with $f \in \cF^\cI$.
In our running example,
the fluent $s$ is considered false by default, that is, the following rule:
\begin{IEEEeqnarray}{c C l}
\sneg s &\leftarrow& \neg s
	\label{eq:pink.8}
\end{IEEEeqnarray}
sating that, unless $s$ is proved, we should considerer that $\sneg s$ holds, is added to the program.
The initial state corresponding with Example~\ref{ex:pink.simple},
would be represented by the \emph{initial formula}:
% \footnote{In the syntax of~\cite{CabalarKSS18}, this initial formula is actually written $\initially \to (\sneg v \wedge \sneg l \wedge r)$.}:
\begin{gather}
\sneg v_0 \wedge \sneg l_0 \wedge r_0 
	\label{eq:pink.simple.initial}
\end{gather}
where the subindex in each literal states that the formula holds at the initial state.
In other words, a temporal atom of the form $a_i$ means that atom $a$ holds at state~$i$.
We can then use the program
$\Pi_{\mathit{pink}}$
containing \mbox{rules~\eqref{eq:pink.1}-\eqref{eq:pink.8}}
to obtain that
\mbox{$\pi_{simple} = \den{\move;\taker}$}
is a valid plan to obtain the diamond in Example~\ref{ex:pink.simple}.

 \comment{Put this program in the syntax of telingo in a Figure?}
 \comment{talk about epistemic specifications and conformant plan here}



% That is,
% Let $\Pi_{\mathit{pink}}$
% % = \set{\eqref{eq:pink.1}-\eqref{eq:pink.5}}$
% be the temporal logic program containing rules~\eqref{eq:pink.1}-\eqref{eq:pink.8}.
% Then, we can use this program for different reasoning tasks in this domain, like prediction or planning.
% For instance, we can see that program
% $$\newprogram\label{prg:pink.simple.prediction} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.simple.initial}} \cup \set{\At{1}{\move} \wedge \At{2}{\taker} }$$
% has a unique temporal stable model $T_{\ref{prg:pink.simple.prediction}}$ of length~$3$, and this satisfies the formula:
% \begin{gather}
% (\sneg v_0 \wedge r_0 \wedge \sneg d_0) \wedge (v_1 \wedge r_1 \wedge \sneg d_1) \wedge (v_2 \wedge r_2 \wedge d_2)
% 	\label{eq::pink.simple.model}
% \end{gather}
% In other words, after moving, the thief is inside the vault without the diamond and, after taking what is in the right pedestal, she is still inside the vault, but now holding the diamond.
% Interestingly,
% we can use a slight variation of program~\program\ref{prg:pink.simple.prediction} to obtain a plan to achieve a certain goal, in our case being in possession of diamond~($d$).
% Let $\Pi_{\mathit{choice}}$ be the program containing a rule of the form $a \vee \neg a$ for each action
% $a \in \set{\move , \flick , \takel , \taker}$.
% Note that, in contrast with classical logic, the formula $a \vee \neg a$ corresponding with the exclude middle axiom is not a tautology under the stable model semantics.
% In fact $a \vee \neg a$ allow us to chose whether $a$ holds or not, instead of assuming that by default it does not hold.
% Then, the program
% $$\newprogram\label{prg:pink.simnple.planning} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.simple.initial}} \cup \Pi_{\mathit{choice}} \cup \set{ \finally(\neg\neg d) }$$
% also has $T_{\ref{prg:pink.simple.prediction}}$ as its unique temporal stable model of length~$3$
% and we have that this model satisfies
% $\At{1}{\move} \wedge \At{2}{\taker}$.
% Note that, in contrast with program~\program\ref{prg:pink.simple.prediction},
% now we have not specify any sequence of actions, but replace it by the program~$\Pi_{\mathit{choice}}$ which give us the possibility of choosing any possible sequence of actions.
% Then, the constraint $\finally(\neg\neg d)$ ensures that every temporal stable model of $\program\ref{prg:pink.simnple.planning}$ satisfies that the thief is holding the diamond~($d$) at its final situation.
% Note again, that in contrast with classical logic, $\neg\neg d$ is not equivalent to $d$ and, in fact, it states that $d$ must hold but without providing any support for this claim. Then, the support for $d$ must come from the rest of the program and, in particular, from the actions chosen in the model.
% This ensures that the sequence of actions $\tuple{\move,\taker}$ is in fact a plan that achieves $d$.

% Let us now consider the initial state laid out in Example~\ref{ex:pink}, that is, that the thief does not know whether the diamond is in the right or left pedestal.
% In this case, the initial situation can be stated by the formula:
% \begin{gather}
% \sneg v_0 \wedge \sneg l_0 \wedge (r_0 \vee \sneg r_0)
% 	\label{eq:pink.initial}
% \end{gather}
% where we have just replace $r_0$ in~\eqref{eq:pink.simple.initial} by $r_0 \vee \sneg r_0$.
% That is, the fact that the thief knows that the Pink Panther is in the right pedestal by the fact that she does not know whether it is in the right or left pedestal.
% Let us now consider the program:
% $$\newprogram\label{prg:pink.prediction} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.initial}} \cup \set{\At{1}{\move} \wedge \At{2}{\taker} }$$
% obtained by replacing, in program~\program\ref{prg:pink.simple.prediction}, the initial formula~\eqref{eq:pink.simple.initial} by the formula~\eqref{eq:pink.initial} representing the new initial state.
% This program has two temporal stable models of length~$3$, namely $T_{\ref{prg:pink.simple.prediction}}$ and $T_{\ref{prg:pink.prediction}}$, where $T_{\ref{prg:pink.simple.prediction}}$ is exactly the same temporal stable model of program~\program\ref{prg:pink.simple.prediction} and, thus, satisfies the formula~\eqref{eq::pink.simple.model}.
% On the other hand, the model $T_{\ref{prg:pink.prediction}}$ satisfies the formula:
% \begin{gather}
% (\sneg v_0 \wedge \sneg r_0 \wedge \sneg d_0) \wedge (v_1 \wedge \sneg r_1 \wedge \sneg d_1) \wedge (v_1 \wedge \sneg r_1 \wedge \sneg d_1)
% 	\label{eq::pink.model}
% \end{gather}
% In other words, model
% $T_{\ref{prg:pink.simple.prediction}}$
% represents the possible evolution of the world in the case that the diamond is in the right pedestal, while
% $T_{\ref{prg:pink.prediction}}$
% represents the evolution of the world in the case that the diamond is in the left one.
% Accordingly,
% in
% $T_{\ref{prg:pink.simple.prediction}}$ the thief achieves the goal of taking the diamond, while in
% $T_{\ref{prg:pink.prediction}}$ she does not.
% We can say that 
% $\tuple{\move,\taker}$ is a \emph{weak plan} of the scenario set out in Example~\ref{ex:pink} in the sense that it may achieve~$d$ in some situations, but not a \emph{strong plan}\footnote{A strong plan is also usually call a conformant plan.} in the sense that achieving the goal is not guaranteed.
% We can also consider now the program
% $$\newprogram\label{prg:pink.prediction2} \quad\eqdef\quad \program\ref{prg:pink.prediction} \cup \set{\At{3}{\takel} }$$
% which has two stable models of length~4,
% namely $T_{\ref{prg:pink.simple.prediction}}'$ and $T_{\ref{prg:pink.prediction}}'$,
% which respectively extend models $T_{\ref{prg:pink.simple.prediction}}$ and $T_{\ref{prg:pink.prediction}}$
% as follows:
% $T_{\ref{prg:pink.simple.prediction}}'$ satisfies the formula~$\eqref{eq::pink.simple.model} \wedge (v_3 \wedge r_3 \wedge  d_3)$
% while
% $T_{\ref{prg:pink.prediction}}'$ satisfies the
% formula~$\eqref{eq::pink.model} \wedge (v_3 \wedge \sneg r_3 \wedge  d_3)$.
% Note that in both cases, $d$ holds at the final situation, that is, after trying to take whatever is in both, the right and left pedestals, we can be sure the thief has achieve the goal of possessing the diamond.
% In this sense, we can say that $\tuple{\move,\taker,\takel}$ is a strong plan for this scenario.

% Let us now try to obtain the plans for this scenario with the same slightly modification we use with Example~\ref{ex:pink.simple}, so we define the program
% $$\newprogram\label{prg:pink.planning} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.initial}} \cup \Pi_{\mathit{choice}} \cup \set{ \finally(\neg\neg d) }$$
% which has two temporal stable model of length~3, namely $T_{\ref{prg:pink.simple.prediction}}$ and 
% $T_{\ref{prg:pink.planning}}$ where
% $T_{\ref{prg:pink.planning}}$ is the symmetric counterpart of model $T_{\ref{prg:pink.simple.prediction}}$ in which the diamond is initially in the left pedestal and that chosen action is $\takel$.
% There are also \comment{add here the number} temporal stable model of length~4, among which we have
% $T_{\ref{prg:pink.simple.prediction}}'$ and $T_{\ref{prg:pink.prediction}}'$.
% Note that, while the two temporal stable models of length~3 represent two different weak plans, the models
% $T_{\ref{prg:pink.simple.prediction}}'$ and $T_{\ref{prg:pink.prediction}}'$ represent the same strong plan.
% In other words, we can compute the weak plans of scenarios involving non-determinism using standard ASP, but there is not direct way of representing that a sequence of actions is a strong plan.
% Of course, we can take a weak plan obtained by this method and check whether it is a strong plan by using the prediction model and check whether all possible states lead to final states that satisfy the goal.

% On the other hand, a more direct and elegant way of obtaining strong plans is using the language of \emph{epistemic specifications}~\cite{Gelfond91}.
% This language was latter generalised to a full logical language~\comment{add cite} containing the modal operator~$\bL$
% that allows us writing formulas of the form $\bL \varphi$ to express that ``$\varphi$ is believed.''
% Using this language, we can obtain the strong plans of Example~\ref{ex:pink} by using the following program:
% $$\newprogram\label{prg:pink.strong.planning} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.initial}} \cup \Pi_{\bL\!\mathit{choice}} \cup \set{ \bL\finally(\neg\neg d) }$$
% where $\Pi_{\bL\!\mathit{choice}}$ is the program containing a rule of the form \mbox{$\bK a \vee \bK \neg a$} for each action
% $a \in \set{\move , \flick , \takel , \taker}$
% and where $\bK$ is a modality corresponding to the reflexive closure of $\bL$, that is,
% we have
% $\bK \varphi \eqdef \varphi \wedge \bL \varphi$ stands for ``$\varphi$ is known.''
% This program has no \emph{temporal world view}, set of temporal stable models, of length~$3$ and two \emph{temporal world view} of length~$4$ which correspond to the strong plans
% $\tuple{\move,\taker,\takel}$
% and
% $\tuple{\move,\takel,\taker}$.
% We also can obtain the weak plans of corresponding to Example~\ref{ex:pink} with the program
% $$\newprogram\label{prg:pink.strong.planning} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.initial}} \cup \Pi_{\bL\!\mathit{choice}} \cup \set{ \bM\finally(\neg\neg d) }$$
% where $\bM \varphi \eqdef \neg\!\bL\!\neg\varphi$ means that ``$\varphi$ is possible.''
% In this case, there is for instance a temporal world view of length~3 containing the two temporal stable models
% $T_{\ref{prg:pink.simple.prediction}}$ and $T_{\ref{prg:pink.prediction}}$ of program~\program\ref{prg:pink.prediction}.



% Before consider the Example~\ref{ex:pink} in its full extension, let us discuss an intermediate step between Examples~\ref{ex:pink.simple} and~\ref{ex:pink}.


% \begin{examplecont}{ex:pink}\label{ex:pink.light}
% Consider now the same initial state as in Example~\ref{ex:pink} but where the thief knows that the light inside the vault is on.\qed
% \end{examplecont}

% As in our previous scenario, the thief may take whatever is on both pedestals and be sure she gets the diamond.
% On the other hand, in this scenario, the thief may also reason that, since the light is on, she would see~($s$) where the diamond is once she enters the vault.
% That is, we have that with the initial state
% \begin{gather}
% \sneg v_0 \wedge l_0 \wedge (r_0 \vee \sneg r_0)
% 	\label{eq:pink.initia.light}
% \end{gather}
% we have that program:
% $$\newprogram\label{prg:pink.prediction.light} \quad\eqdef\quad \Pi_{\mathit{pink}} \cup \set{ \eqref{eq:pink.initia.light} } \cup \set{\At{1}{\move} }$$
% has two stable models satisfying formulas $v_1 \wedge l_1 \wedge r_1 \wedge s_1$
% and
% $v_1 \wedge l_1 \wedge \sneg r_1 \wedge s_1$.
% In this sense, she could also reason that, though right now she does not know whether the Pink Panther is on the left or right pedestal, she will discover this fact as soon as she enters the vault and sees ($s$) it.
% Accordingly, she may develop a \emph{conditional plan} for this situation in which first she moves inside the vault and then she takes whatever is in the right or left pedestal depending on whether she sees that the diamond is in one or the other.
% It is now easy to see that the thief may develop a similar conditional plan for Example~\ref{ex:pink} in which she $\flick$ the light just after moving inside the vault.
% Unfortunately, there is no clear way to represent this neither using standard ASP nor the language of epistemic specifications.



% On the other hand, a way to obtain the conditional plans of our running example may consist in using Dynamic Epistemic Logic (DEL)~\cite{BatlagMS98}, a methodology that was developed in~\mbox{\cite{AndersenBJ12,BolanderA11,Bolander17}}.
% According to this methodology, the state of the world is represented as \emph{epistemic models}.
% For instance, Figure~\ref{fig:pink.state1}a
% represents an state where the thief is in the vault with the light of and where she does not know whether the Pink Panther is on the right or left pedestal.
% This state corresponds to the propositional formula~$v \wedge \sneg l \wedge (r \vee \sneg r)$ in ASP.
% \begin{figure}
% \begin{center}
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1: v\underline{l}r$] {};
% \node[point] (v) [label=below:$w_2 :v\underline{lr}$,right=of w] {};
% \path[-] (w) edge (v);
% \end{tikzpicture}
% \\
% (a)
% \end{center}
% \end{minipage}
% \hspace{0.25cm}
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1: v\underline{l}r$] {};
% \node[point] (v) [label=below:$w_2 :v\underline{lr}$,right=of w] {};
% \end{tikzpicture}
% \\
% (b)
% \end{center}
% \end{minipage}
% \end{center}
% 	\caption{ (a) Epistemic model corresponding to state where the thief is in the vault with the light of and where she does not know whether the Pink Panther is on the right or left pedestal.
% 	(b) Epistemic model corresponding to state where the thief is in the vault with the light of and where she does know whether the Pink Panther is on the right or left pedestal.
% 	We use $\underline{p}$ to represent that proposition $p$ is false in some world.
% 	The path between $w_1$ and $w_2$ in (a) means that these two worlds are will not distinguishable for the thief at that state.
% 	}\label{fig:pink.state1}
% \end{figure}
% For the sake of comparative Figure~\ref{fig:pink.state1}b depicts an alternative epistemic model in which the truth of each proposition in each world is the same, but in which the thief actually knows whether the Pink Panther is on the right or left pedestal.
% This epistemic model cannot be represented by any propositional formula in ASP, but it corresponds to the formula $v \wedge \sneg l \wedge (\bK r \vee \bK \sneg r)$ in the language of epistemic specifications.
% Note, however, that this knowledge correspond to the knowledge that the thief will have while carrying the plan on, not to the knowledge she has at the moment she is developing the plan.
% Following terminology from~\cite{BolanderA11}, we can say that worlds~$w_1$ and~$w_2$ are \emph{run-time distinguishable} in (b), but \emph{planning-time indistinguishable}. In (a), worlds~$w_1$ and~$w_2$  run-time and planning-time indistinguishable, that is, the thief is not able to distinguish between these two possible worlds neither when making the plan nor when carrying it on.



% From a knowledge representation point of view,
% a key difference between the use of ASP and DEL in representing these dynamic domains is how the effects of actions are represented:
% through logic programs in the case of ASP and through \emph{event models}~\cite{van2008semantic} in the case of DEL.
% As we already have seen, logic programs are logical theories of a particular shape.
% On the other hand, roughly speaking, an event model consists of a \emph{Kripke frame}
% and an mapping associating to each world some preconditions and postconditions.
% Figure~\ref{fig:pink.actions} contains the event models taken from~\cite{AndersenBJ12} that correspond to the actions of Example~\ref{ex:pink}.
% \begin{figure}
% \includegraphics[width=\textwidth]{actions.png}
% 	\caption{Event models representing the actions of the thief in Example~\ref{ex:pink}.}
% 	\label{fig:pink.actions}
% \end{figure}
% For instance, we can see that the action $\takel$ consists of a single world whose precondition $v \wedge \sneg d$ state that is only applicable if the thief is in the vault and she does not have the diamond; and whose postcondition $\set{d \mapsto \sneg r}$ states that $d$ is true if and only if $\sneg r$ previously hold.
% More interestingly, is the action $\flick$ which has two isolated worlds with the same postcondition $\set{ l \mapsto \top }$, which states that the light will turn on, but with different preconditions that correspond to the cases in which thief is in the vault and the Pink Panther is on the right ($r \wedge v$) or the left ($\sneg r \wedge v$) pedestal, receptively.
% The fact that these two worlds are isolated encodes that these two events are distinguishable for the agent after performing the action.
% To further illustrate this point, let us consider the result of performing the action $\flick$ in the epistemic model of Figure~\ref{fig:pink.state1}a.
% After \emph{updating} this epistemic model with the event model corresponding to the action $\flick$ 
% we obtain the epistemic model of Figure~\ref{fig:pink.state2}.
% \begin{figure}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1' : vlr$] {};
% \node[point] (v) [label=below:$w_2' :vl\underline{r}$,right=of w] {};
% \end{tikzpicture}
% \end{center}
% 	\caption{Epistemic model obtained after updating the model of Figure~\ref{fig:pink.state1} with the event model corresponding to the action $\flick$.}\label{fig:pink.state2}
% \end{figure}
% Note that each $w_i'$ has the same evaluation as $w_i$ but with $l$ being true.
% On the other hand, $w_1'$ and $w_2'$ are not connected in Figure~\ref{fig:pink.state2}
% while $w_1$ and $w_2$ where connected.
% This means that after performing the action $\flick$
% the two previous runt-time indistinguishable possible worlds become run-time distinguishable.
% For the sake of comparative, consider now an action $\flick'$ which is as $\flick$ but with worlds $e_1$ and $e_2$ connected.
% Then, the result of updating the epistemic model of Figure~\ref{fig:pink.state1}a
% with the event model of $\flick'$ is depicted Figure~\ref{fig:pink.state3}.
% \begin{figure}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1' : vlr$] {};
% \node[point] (v) [label=below:$w_2' :vl\underline{r}$,right=of w] {};
% \path[-] (w) edge (v);
% \end{tikzpicture}
% \end{center}
% 	\caption{Epistemic model obtained after updating the model of Figure~\ref{fig:pink.state1} with the event model corresponding to the action $\flick$.}\label{fig:pink.state3}
% \end{figure}
% Note that the valuations of each world in Figures~\ref{fig:pink.state2} and~\ref{fig:pink.state3} is the same, but now worlds $w_1'$ and $w_2'$ are connected.
% This means that they did not become run-time distinguishable after performing the action $\flick'$.
% In this sense, action $\flick'$ could be intuitively understood as an action that turns on the light but that does not allow to see the pedestals, it may be because they are hide behind a curtain, because the thief is not looking the the direction of the pedestals...
% Finally, let us pay attention to the action~$\move$,
% which has three worlds with the same postcondition $\set{v \mapsto \neg v}$ stating that it flips the value of $v$.
% On the other hand, each of the worlds has different preconditions meaning that they are applicable in different circumstances.
% The precondition of the first $v \vee (\neg v \wedge \neg l)$ means that is applicable when we are inside the vault or outside with the light off.
% For instance, it easy to see that this is the only precondition among the worlds of $\move$ that hold in every world of the epistemic model corresponding to the initial state of Example~\ref{ex:pink}, which is depicted in Figure~\ref{fig:pink.state0}a.
% \begin{figure}
% \begin{center}
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1 : \underline{vl}r$] {};
% \node[point] (v) [label=below:$w_2 : \underline{vlr}$,right=of w] {};
% \path[-] (w) edge (v);
% \end{tikzpicture}
% \\
% (a)
% \end{center}
% \end{minipage}
% \hspace{0.25cm}
% \begin{minipage}{0.4\textwidth}
% \begin{center}
% \begin{tikzpicture}[align=center,node distance=2cm]
% \node[point] (w) [label=below:$w_1 : \underline{v}lr$] {};
% \node[point] (v) [label=below:$w_2 : \underline{v}l\underline{r}$,right=of w] {};
% \path[-] (w) edge (v);
% \end{tikzpicture}
% \\
% (b)
% \end{center}
% \end{minipage}
% \end{center}
% 	\caption{(a) Epistemic model corresponding to the initial state of Example~\ref{ex:pink}. (b) Epistemic model corresponding to a variation in which the light is initially on.}\label{fig:pink.state0}
% \end{figure}
% As a result, applying the action~$\move$ to the epistemic model in Figure~\ref{fig:pink.state0}a, only changes the value of~$v$, leading to the epistemic model in Figure~\ref{fig:pink.state1}.
% On the other hand, if we apply the action $\move$ to the alternative epistemic model of Figure~\ref{fig:pink.state0}b, in which the light is initially on, we have that~$w_1$ satisfies the preconditions of $f_2$
% while $w_2$ satisfies the preconditions of $f_3$.
% As a result, after applying the action $\move$, we obtain the epistemic model of Figure~\ref{fig:pink.state1}b.
% In other words, after moving into the vault with the light turned on, the thief has knowledge about whether the Pink Panther is on the right or left pedestal.

% Despite the representational power of event models to represent actions, this example illustrates one of its clear limitations:
% defining event model from the informal description of an action is far from trivial~\cite{Bolander17}.
% As discussed in~\cite{Bolander14}, one of the reasons for this difficulty is that an event model need to hardcode both the effects of the action into the world and the information gained from observing the effects of this action.
% Note that, in the informal description of Example~\ref{ex:pink}, the  fact
% \emph{``if the thief is in the vault ($v$) and the light is on ($l$), the thief can see~($s$) where the Pink Panther is''} is not expressed as a direct effect of any action, but a indirect effect triggered by the a state satisfying the condition $v \wedge l$.
% However, when this is encoded as event models, we have that this piece of
% knowledge is included as direct effects of the actions $\flick$ and $\move$, which are the actions affecting the values of $v$ and $l$.
% This is a clear manifestation of well-known \emph{ramification problem}~\comment{add cite}.

% ASP is well-know for its knowledge representation versatility and, in fact, it is a formalism well-capable of representing indirect effects~\comment{add cite}.
% On the other hand, we have already seen that it lacks the expressibility to represent conditional planning.
% This motivate us to develop a new formalism, we call it Dynamic Epistemic ASP (DEASP), that combines the knowledge representation capabilities of ASP with DEL capabilities of reasoning with knowledge and develop conditional plans.
% In fact, as we will see latter, Example~\ref{ex:pink}, can be represented in DEAS by adding the rule
% \begin{gather}
% \bO r \leftarrow s
% 	\label{eq:pink.obs}
% \end{gather}
% to the program~$\Pi_{pink}$.
% Informally, rule~\eqref{eq:pink.obs} can be read as ``$r$ is observed whenever $l$ and $v$ hold.''







==> outline.tex <==
%!TEX root = main.tex
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

\renewcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}
\renewcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}
\renewcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}
\renewcommand{\final}{\ensuremath{\mbox{\outline{$\bm{\mathsf{f}}$}}}}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

